Opaque Service Virtualisation: A Practical Tool for Emulating Endpoint Systems

Large enterprise software systems make many complex interactions with other services in their environment. Developing and testing for production-like conditions is therefore a very challenging task. Current approaches include emulation of dependent services using either explicit modelling or record-and-replay approaches. Models require deep knowledge of the target services while record-and-replay is limited in accuracy. Both face developmental and scaling issues. We present a new technique that improves the accuracy of record-and-replay approaches, without requiring prior knowledge of the service protocols. The approach uses Multiple Sequence Alignment to derive message prototypes from recorded system interactions and a scheme to match incoming request messages against prototypes to generate response messages. We use a modified Needleman-Wunsch algorithm for distance calculation during message matching. Our approach has shown greater than 99% accuracy for four evaluated enterprise system messaging protocols. The approach has been successfully integrated into the CA Service Virtualization commercial product to complement its existing techniques.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}




==> edits <==
The core contribution of our approach is a method to formulate a
representative cluster prototype. This step consists of three major
subparts: (1) aligning the commong features of the request messages in
a cluster, (2) extracting the common features while accommodating
variations to derive the prototype, and (3) weighting sections of
the prototype according to their relative importance through an
entropy analysis.

\item[A3] We derive a \emph{request consensus prototype} for each operation type cluster, using multiple sequence alignment and extracting the common patterns.

a weightings array, $\mathbf{w}$, of the same length as the prototype $\mathbf{p}$.



==> timing.tex <==
% Document Type: LaTeX
% Master File: timing.tex
% Author: Jean-Guy Schneider
% Last Modified: Fri Sep 5 2014, 14:32

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\resgentime}{
    \begin{tabular}{|>{\centering\arraybackslash}m{0.8cm} |c|>{\centering\arraybackslash}m{1.1cm} |>{\centering\arraybackslash}m{1.1cm} |>{\centering\arraybackslash}m{1.5cm} |>{\centering\arraybackslash}m{1cm}|}
        \hline
      % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
       &No.& Whole Library  & Cluster Centroid & Consensus +Weighting & Real System \\\hline\hline
      IMS  &800& 432 & 4.39 & 2.86 & 518 \\ \hline
      LDAP &2177& 781 & 2.11 & 2.23 & 28  \\ \hline
      LDAP text(1) &2177 & 1176.1 & 5.64 & 6.83 & 28 \\ \hline
      LDAP text(2) &1000& 91.29 & 1.40 & 1.31 & 28 \\ \hline
      SOAP &1000& 328.79 & 2.90 & 3.07 & \\ \hline
      Twitter&1825& 419.82 & 48.84 & 49.45 & 417 \\ \hline
    \end{tabular}
}
\newcommand{\matchingtime}{
 \resizebox{0.49\textwidth}{!}{
    \begin{tabular}{|>{\centering\arraybackslash}m{0.8cm} |c|>{\centering\arraybackslash}m{0.8cm} |>{\centering\arraybackslash}m{0.6cm} |>{\centering\arraybackslash}m{0.6cm} 
    |>{\centering\arraybackslash}m{0.6cm} |>{\centering\arraybackslash}m{0.6cm} |>{\centering\arraybackslash}m{0.6cm} |}
  
   % \begin{tabular}{|c|c|c|c|c|c|c|c|}
        \hline
      % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
       \multirow{2}{0.5cm}{}&\multirow{2}{0.5cm}{\centering No.}& \multicolumn{2}{c|}{\multirow{1}{*}{Whole Library}}  & \multicolumn{2}{c|}{\multirow{1}{*}{Cluster Centroid}} & \multicolumn{2}{c|}{Consensus+W} \\\cline{3-8}
       &&M&S&M&S&M&S \\\hline\hline
      \multirow{1}{0.5cm}{IMS} &800& 431.43 & 0.41 & 3.35 & 0.98 & 2.31 & 0.61 \\ \hline
      LDAP &2177& 771.54 & 6.28 & 1.58 & 0.27 & 2.03 & 0.21 \\ \hline
      LDAP text(1) &2177 & 1174.81 & 1.18 & 4.31 & 1.17 & 5.37 & 1.33 \\ \hline
      LDAP text(2) &1000& 91.17 & 4.18 & 0.77 & 0.64 & 0.96 & 0.35 \\ \hline
      SOAP &1000& 330.38 & 1.19 & 1.88 & 0.97  & 2.16 & 0.87 \\ \hline
      Twitter &1825& 352.65 & 51.11& 0.86 & 48.03 & 1.23 & 48.29 \\ \hline
    \end{tabular}
 }   
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% Original Tables %%%%

% \newcommand{\resgentime}{
%     \begin{tabular}{|>{\centering\arraybackslash}m{0.8cm} |c|>{\centering\arraybackslash}m{1.1cm} |>{\centering\arraybackslash}m{1.1cm} |>{\centering\arraybackslash}m{1.5cm} |>{\centering\arraybackslash}m{1cm}|}
%         \hline
%       % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
%        &No.& Whole Library  & Cluster Centroid & Consensus +Weighting & Real System \\\hline\hline
%       IMS  &800& 470.99 & 4.94 & 3.24& 518\\ \hline
%       LDAP &2177& 835.91 & 2.77 & 2.88 & 28  \\ \hline
%       LDAP text(1) &2177 & 1434.70 & 5.69 & 7.30 & 28 \\ \hline
%       LDAP text(2) &1000& 266.30 & 2.44 & 1.63 & 28 \\ \hline
%       SOAP &1000& 380.24 & 2.97 & 3.35 & \\ \hline
%       Twitter&1825& 464.09 & 32.86 & 36.62 & 417 \\ \hline
%     \end{tabular}
% }
% \newcommand{\matchingtime}{
%  \resizebox{0.49\textwidth}{!}{
%     \begin{tabular}{|>{\centering\arraybackslash}m{0.8cm} |c|>{\centering\arraybackslash}m{0.8cm} |>{\centering\arraybackslash}m{0.6cm} |>{\centering\arraybackslash}m{0.6cm} 
%     |>{\centering\arraybackslash}m{0.6cm} |>{\centering\arraybackslash}m{0.6cm} |>{\centering\arraybackslash}m{0.6cm} |}
  
%    % \begin{tabular}{|c|c|c|c|c|c|c|c|}
%         \hline
%       % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
%        \multirow{2}{0.5cm}{}&\multirow{2}{0.5cm}{\centering No.}& \multicolumn{2}{c|}{\multirow{1}{*}{Whole Library}}  & \multicolumn{2}{c|}{\multirow{1}{*}{Cluster Centroid}} & \multicolumn{2}{c|}{Consensus+W} \\\cline{3-8}
%        &&M&S&M&S&M&S \\\hline\hline
%       \multirow{1}{0.5cm}{IMS} &800& 460.78&10.2 & 3.67 &1.27 & 2.68&0.56 \\ \hline
%       LDAP &2177& 828.95 & 6.96 & 2.38 &0.39& 2.60&0.28 \\ \hline
%       LDAP text(1) &2177 & 1425.23 &9.47& 4.38&1.31 & 5.67&1.63 \\ \hline
%       LDAP text(2) &1000& 257.92 &8.38& 1.35 &1.09& 1.14 &0.49\\ \hline
%       SOAP &1000& 372.58 &7.66& 1.92 &1.05 & 2.45 &0.9\\ \hline
%       Twitter &1825& 412.98 &51.11& 1.47 &31.39& 1.67 &34.95 \\ \hline
%     \end{tabular}
%  }   
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

